Achieving Maximin Share and EFX/EF1 Guarantees Simultaneously

We study the problem of computing \emph{fair} divisions of a set of indivisible goods among agents with \emph{additive} valuations. For the past many decades, the literature has explored various notions of fairness, that can be primarily seen as either having \emph{envy-based} or \emph{share-based} lens. For the discrete setting of resource-allocation problems, \emph{envy-free up to any good} (EFX) and \emph{maximin share} (MMS) are widely considered as the flag-bearers of fairness notions in the above two categories, thereby capturing different aspects of fairness herein. Due to lack of existence results of these notions and the fact that a good approximation of EFX or MMS does not imply particularly strong guarantees of the other, it becomes important to understand the compatibility of EFX and MMS allocations with one another. In this work, we identify a novel way to simultaneously achieve MMS guarantees with EFX/EF1 notions of fairness, while beating the best known approximation factors [Chaudhury et al., 2021, Amanatidis et al., 2020]. Our main contribution is to constructively prove the existence of (i) a partial allocation that is both $2/3$-MMS and EFX, and (ii) a complete allocation that is both $2/3$-MMS and EF1. Our algorithms run in pseudo-polynomial time if the approximation factor for MMS is relaxed to $2/3-\varepsilon$ for any constant $\varepsilon > 0$ and in polynomial time if, in addition, the EFX (or EF1) guarantee is relaxed to $(1-\delta)$-EFX (or $(1-\delta)$-EF1) for any constant $\delta>0$. In particular, we improve from the best approximation factor known prior to our work, which computes partial allocations that are $1/2$-MMS and EFX in pseudo-polynomial time [Chaudhury et al., 2021].

==> comparison-aaai.tex <==
%\section{\boldmath Relations Between $\efx$/$\ef1$ and $\mms$} \label{sec:relation}

Now we briefly discuss the guarantees $\efx$/$\ef1$ allocations can provide for $\mms$ and vice versa. \citet{comparing-efx} gave a comprehensive comparison between these notions of fairness. Here we mention a few.
%In particular, they proved that while a complete $\efx$ allocation implies $4/7$-$\mms$ guarantee, there exists complete $\efx$ allocations which are as bad as $0.5914$-$\mms$. Nevertheless, these guarantees become relevant only when a complete $\efx$ allocation exists which, in itself, is a big open problem. 
\begin{proposition}[\citet{comparing-efx}]
    For arbitrary $n \geq 1$, any $\efx$ allocation is also a $4/7$-$\mms$ allocation. On the other hand, an $\efx$ allocation is not necessarily an $\alpha$-$\mms$ allocation for $\alpha>0.5914$ and large enough $n$.
\end{proposition}

%In this work, we show that the relation is even weaker between $\ef1$ and $\mms$. Furthermore, we show that, for any $\alpha>0$, $\alpha$-$\mms$ allocations do not guarantee any bounded approximation ratio for $\ef1$ and hence also $\efx$. 
%The proofs of following propositions can be found in Appendix~\ref{app:missing-proofs}.

\begin{restatable}[\citet{comparing-efx}]{proposition}{propone}
    An $\ef1$ allocation is not necessarily an $\alpha$-$\mms$ allocation for any $\alpha>1/n$.
\end{restatable}


\begin{restatable}{proposition}{proptwo}
    For $n \geq 3$ and any $\alpha>0$, an $\alpha$-$\mms$ allocation is not necessarily $\beta$-$\ef1$ for any $\beta > 0$.
\end{restatable}

Therefore, we can conclude that, by guaranteeing one of approximate $\mms$ or approximate $\efx$/$\ef1$, one cannot obtain a good guarantee for the other notion of fairness for free. 





%In Section \ref{sec:limitations} \todo{...}, we discuss other existing algorithms to compute either of $2/3$-$\mms$ or $\efx$/$\ef1$, where none of these algorithms guarantee the other fairness criterion. This suggests that while guaranteeing each of these fairness notions (besides $\ef1$) is difficult on its own, satisfying both kinds of fairness guarantees simultaneously becomes an even more challenging problem.

==> limitations.tex <==
\section{Limitations of the Existing Approaches}\label{sec:limitations}
%In this section, we discuss that all the known algorithms which output a $2/3$-$\mms$ allocation, do not guarantee $\efx$ or $\ef1$ property. Similarly, all the known algorithms which output an $\ef1$ or a partial $\efx$ allocation, do not guarantee any bound better than $1/2$-$\mms$. 

\todo{Except \cite{kurokawa2018fair} and \cite{amanatidis2017approximation}, all approx $\mms$ algorithms rely on ordered instances which does not guarantee anything for the actual instance. And these two use our approach which remove agents after they are $2/3$-$\mms$ satisfied and thus not guarantee any fairness criteria.}

==> technical.tex <==
\section{Technical Overview} \label{sec:tech_overview}
In this section, we give a high-level overview of the techniques used in this work. The first contribution of our work is an alternative approach for computing $2/3$-$\mms$ allocations in Section~\ref{sec:mms}. Surprisingly, it does \emph{not} rely on the two most common tools on computing approximate $\mms$ allocations, namely \emph{ordered instances} and \emph{valid reductions}. Let us first briefly describe these tools.

\paragraph{Ordered Instances.} We say that a fair division instance is \emph{ordered} if we can rename the goods such that $v_i(g_1) \geq \ldots \geq v_i(g_m)$ holds true for all agents $i \in [n]$. \cite{barman2020approximation} showed that, for any $\alpha \in [0,1]$, if $\alpha$-$\mms$ allocations exist for ordered instances, then $\alpha$-$\mms$ allocations exist for all instances. Therefore, it becomes natural to assume ordered instances while studying $\alpha$-$\mms$ allocations, as done by many of the previous works in the literature.

\paragraph{Valid Reductions.} Another common tool in computing $\alpha$-$\mms$ allocations, is valid reductions \citep{}. Allocating a bundle $B$ to an agent $i$ and removing agent $i$ with $B$ from consideration to \emph{reduce} to a smaller instance is said to be \emph{valid}  if
\begin{itemize}
    \item $v_i(B) \geq \alpha \cdot \mms_i$, and
    \item $\mms^{n-1}_j(\M \setminus B) \geq \mms^n_j(\M)$ for all $j \neq i$.
\end{itemize}
In other words, allocating $B$ to agent $i$ is harmless since, not only $B$ satisfies $i$, but also removing $i$ and $B$ from the instance, does not decrease the $\mms$ value of the remaining agents. Hence, one can, without loss of generality, allocate $B$ to $i$ and proceed with computing an $\alpha$-$\mms$ allocation in the reduced instance. 

Unfortunately, none of these tools can be used when dealing with envy-based notions of fairness. And hence, most of the previous works that achieve approximate $\mms$ guarantees do not obtain any envy-based criteria results \cite{}. On the other hand, most of the previous work that achieve simultaneous guarantees for $\mms$ and $\efx$/$\ef1$ are obtained by manipulating algorithms that provide $\efx$/$\ef1$ guarantees so that some approximation for $\mms$ can also be achieved. However, so far, the envy-based algorithmic techniques have not been strong enough to also attain $2/3$-$\mms$ guarantee.

In Section \ref{sec:limitations}, we discuss other existing algorithms to compute either of $2/3$-$\mms$ or $\efx$/$\ef1$, where none of these algorithms guarantee the other fairness criterion. This suggests that while guaranteeing each of these fairness notions (besides $\ef1$) is difficult on its own, satisfying both kinds of fairness guarantees simultaneously becomes an even more challenging problem.

\paragraph{Computing $2/3$-$\mms$ Allocations:} Recently, \cite{AR24eefx} proved that $\eefx$ allocations are guaranteed to exist for fair division instances with general \emph{monotone} valuations. Even though, it does not directly work for our purposes, we are able to carefully modify their technique to compute $2/3$-$\mms$ allocations for instances with additive valuations. The idea is to repeat the following process: in each round with $n'$ remaining agents (initially $n'=n$), compute a partition of the remaining goods into $n'$ many bundles $X_1, \ldots, X_{n'}$ and consider the following bipartite graph $T=(V,E)$. The vertex set $V$ has $n'$ nodes corresponding to $X_1, \ldots, X_{n'}$ on one side and $n'$ nodes corresponding to the remaining agents on another. There exists an edge between bundle $X_j$ and agent $i$, if and only if, $v_i(X_j) \geq (2/3) \mms_i$. If there exists a perfect matching in $T$, then there exists a $2/3$-$\mms$ allocation. If not, we want to compute a non-empty matching such that there exists no edge between an unmatched agent and a matched bundle. The idea is to allocate bundles according to this matching and solve the problem recursively.

It turns out that (unlike computing $\eefx$ in \citep{AR24eefx}) we cannot blindly solve the problem recursively, since removing the agents and bundles according to the matching may not necessarily be a valid reduction and thus the maximin share value of the remaining agents could decrease. However, we prove that, irrespective of how many agents and bundles are removed, the $\mms$ value of no remaining agent decreases by more than a multiplicative factor of $2/3$. 

We now explain our approach for computing $2/3$-$\mms$ allocations. In each round with $n'$ remaining agents, we let a remaining agent $i$ to divide the items into $n'$ bundles $X_1, \ldots, X_{n'}$ of value at least $(2/3)\mms_i$ to her. Then, we find a matching between the bundles and the agents in $T$, such that all matched agents value their bundle at least $2/3$ fraction of their $\mms$ value and all unmatched agent like all the matched bundles less than $2/3$ fraction of their $\mms$ value. If there is any agent remaining, we simply repeat the above process. (see Algorithm \ref{alg:approx-mms} and Theorem~\ref{thm:2-3-mms} in Section~\ref{sec:mms}). 

\paragraph{Achieving $2/3$-$\mms$ along-with $\efx$:}
We first note that, in Algorithm \ref{alg:approx-mms} (and generally in the algorithmic technique of \cite{AR24eefx}), once an agent receives a bundle $X_i$, $X_i$ would be the final bundle that she receives in the algorithm. That is, once agent $i$ receives the bundle $X_i$, she is out of the consideration. This guarantees that agent $i$ will have the same utility $v_i(X_i)$ in the end of the algorithm but it does not guarantee anything about how much $i$ values other bundles $X_j$ and thus, it does not guarantee $\efx$ (or even $\ef1$) property. 

We overcome this barrier by developing Algorithm \ref{alg:approx-mms+efx} in Section~\ref{sec:main}. Here, we again ask a remaining agent $i$ to partition the goods into $n'$ (number of remaining agents) bundles $X_1, \ldots, X_{n'}$ of value at least $(2/3)\mms_i$. Then, we shrink these bundles to guarantee that every remaining agent value all the strict subsets of these bundles less than $2/3$ fraction of their $\mms$ value. After doing so, if there still exists an agent $j$, who was allocated a bundle in previous iterations and who strongly envies one of $X_1, \ldots, X_{n'}$, say $X_j$, we do the following. We find a \emph{most envious agent}, say $a^*$, of bundle $X_j$ and allocate, to $a^*$, a subset of $X_j$ which $a^*$ envies but no agent strongly envies (see Section \ref{sec:prelim} for definitions of most envious agent and strong envy). This way, we are able to guarantee that at each point during the algorithm, the current (partial) allocation among a subset of agents is $\efx$ with a guarantee that these agents hold a bundle that has a value at least $2/3$ fraction of their $\mms$ value. 


We emphasize that the above-described is a new approach for finding $\efx$ allocations. \cite{chaudhury2021little} proved the existence of partial $\efx$ allocations with little charity\footnote{Here, little charity entails that the partial allocation is $\efx$ such that at most $n-1$ items go to charity and no agent envies this pool of charity.}, by developing an algorithm which starting from an empty allocation, maintains the $\efx$ property at all time steps. While the charity is not small enough (both in size and value), they prove they can alter the current partial $\efx$ allocation to get another (partial) $\efx$ while improving certain potential function. This approach was also used in \citep{}. \cite{AkramiACGMM23} introduced another approach which solved the existence of $\efx$ allocations for $3$ agents with valuation functions more general than additive. Here, the focus is to maintain the property that the allocation is complete and while the allocation is not $\efx$, they alter it to obtain another complete allocation, while (again) improving certain potential function. This approach was used in \citep{} as well. 

To the best of our knowledge, none of the previous algorithms computing an $\efx$ allocation allocates a bundle to some of the agents and nothing to the rest in an intermediate step. It might also seem counter-intuitive to do so, since we need to guarantee that there are enough items left to satisfy the agents who have received nothing so far. We are able to make it possible in Algorithm~\ref{alg:approx-mms+efx}, since we know that all the remaining agents (who have not yet received anything) value all the already allocated bundles less than $2/3$ fraction of their $\mms$ value. Interestingly enough, the share-based guarantee that we are maintaining helps us to prove envy-based guarantees as well. 

\todo{poly-time: we give PTAS. \cite{chaudhury2020efx} prove the existence of (partial) $\efx$ with $1/2$-$\mms$ but it is not poly-time. They can only get poly-time if they have $(1-\epsilon)$-$\efx$ instead of $\efx$. So even computing $1/2$-$\mms$ with $\efx$ in poly-time was open.}


